Machine Learning Methods for Automated Interstellar Object Classification with LSST

The Legacy Survey of Space and Time, to be conducted with the Vera C. Rubin Observatory, is poised to revolutionize our understanding of the Solar System by providing an unprecedented wealth of data on various objects, including the elusive interstellar objects (ISOs). Detecting and classifying ISOs is crucial for studying the composition and diversity of materials from other planetary systems. However, the rarity and brief observation windows of ISOs, coupled with the vast quantities of data to be generated by LSST, create significant challenges for their identification and classification. This study aims to address these challenges by exploring the application of machine learning algorithms to the automated classification of ISO tracklets in simulated LSST data. We employed various machine learning algorithms, including random forests (RFs), stochastic gradient descent (SGD), gradient boosting machines (GBMs), and neural networks (NNs), to classify ISO tracklets in simulated LSST data. We demonstrate that GBM and RF algorithms outperform SGD and NN algorithms in accurately distinguishing ISOs from other Solar System objects. RF analysis shows that many derived Digest2 values are more important than direct observables in classifying ISOs from the LSST tracklets. The GBM model achieves the highest precision, recall, and F1 score, with values of 0.9987, 0.9986, and 0.9987, respectively. These findings lay the foundation for the development of an efficient and robust automated system for ISO discovery using LSST data, paving the way for a deeper understanding of the materials and processes that shape planetary systems beyond our own. The integration of our proposed machine learning approach into the LSST data processing pipeline will optimize the survey's potential for identifying these rare and valuable objects, enabling timely follow-up observations and further characterization.

==> latex_utils.tex <==
\usepackage{etoolbox}
\newtoggle{comments} 


% \newcommand{\fakeheader}[1]
% {\vspace{.75mm} \noindent\textbf{#1}~}


\toggletrue{comments}
% \togglefalse{comments}



\iftoggle{comments}{
    \newcommand{\noterc}[1]
    	{{\color{blue}[{\bf Note:} #1]}}
    \newcommand{\notepv}[1]
    	{{\color{orange}[{\bf Note:} #1]}}
    \newcommand{\todo}[1]
    	{{\color{red}[{\bf Todo:} #1]}}	
    \newcommand{\fix}[1]
    	{{\color{red}{\bf}#1}}	
    \newcommand{\cut}[1]
    	{{\color{red}\sout{#1}}}	

    \newcommand{\changerc}[1]{{\color{blue}#1}}
    \newcommand{\changepv}[1]{{\color{orange}#1}}
}{
    \newcommand{\note}[1]{}
    \newcommand{\todo}[1]{}
    \newcommand{\cut}[1]{}
}




